Verifying C11-Style Weak Memory Libraries via Refinement

Deductive verification of concurrent programs under weak memory has thus far been limited to simple programs over a monolithic state space. For scalability, we also require modular techniques with verifiable library abstractions. This paper addresses this challenge in the context of RC11 RAR, a subset of the C11 memory model that admits relaxed and release-acquire accesses, but disallows, so-called, load-buffering cycles. We develop a simple framework for specifying abstract objects that precisely characterises the observability guarantees of abstract method calls. We show how this framework can be integrated with an operational semantics that enables verification of client programs that execute abstract method calls from a library they use. Finally, we show how implementations of such abstractions in RC11 RAR can be verified by developing a (contextual) refinement framework for abstract objects. Our framework, including the operational semantics, verification technique for client-library programs, and simulation between abstract libraries and their implementations, has been mechanised in Isabelle/HOL.

==> composition.tex <==
\section{Client library composition}

While the verification Key to our paper is the observation that one can compose clients and
objects


==> introduction.tex <==
\section{Introduction}


% \bd{Make this shorter.}

% The introduction and adoption of weak memory has meant that in modern
% concurrent programs, threads may observe stale values of each variable
% due to caching effects.

An effective technique for reasoning about weak memory models is to
consider the observations that a thread can make of the
writes % that have occurred
within a system.  For example, for certain subsets of C11 (the 2011 C
standard), % consideration of
reasoning about per-thread observations has led to operational
characterisations of the memory model, high-level predicates for
reasoning about per-thread observations, and deductive verification
techniques applied to standard litmus tests and synchronisation
algorithms~\cite{ECOOP20}.
Current verification techniques are however, focussed on (closed)
programs, and hence % , and hence, comprise reasoning over a single (monolithic)
% state space. % While this is a useful starting point, such
% Such techniques 
do not provide any mechanism for (de)composing clients
and libraries. This problem requires special consideration under weak
memory since the execution of a library
method % can (and in many cases are required to)
may induce synchronisation. That is, a thread's observations of a system
(including of client variables) can change % due to the
% execution
when executing % of
library methods.

This paper addresses several questions surrounding client-library
composition in a weak memory context.

{\bf (1)} {\em How can a client \emph{use} a weak memory library,
i.e., what abstract guarantees can a library provide a client program?}
Prior works~\cite{DongolJRA18,DBLP:conf/popl/BattyDG13} describe
techniques for \emph{specifying} the behaviour of abstract objects,
which are in turn related to their implementations using causal
relaxations of linearizability. % The idea here is that in addition to
% behaviours guaranteed in a sequentially consistent context, 
However, these works do not provide a mechanism for reasoning about
the behaviour of client programs that {\em use} abstract libraries. In
this paper, we address this gap by presenting a modular operational
semantics % and associated verification technique
that combines weak
memory states of clients and libraries.
% Moreover, we develop an operational semantics for showing how
% one can reason about the composition of client-library programs based
% on an abstract library specification.  
This is our first
contribution. 


{\bf (2)} {\em What does it mean to \emph{implement} an abstract
  library?}  To ensure that behaviours of client programs using an
abstract library are preserved, we require \emph{contextual
  refinement} between a library implementation and its abstract
specification. This guarantees that no new client behaviours are
introduced when a client uses a (concrete) library implementation in
place of its (abstract) library specification. Under sequential
consistency (SC), it is well known that linearizable libraries
guarantee (contextual)
refinement~\cite{DBLP:conf/icfem/DongolG16,GotsmanY11,DBLP:journals/tcs/FilipovicORY10}. However,
under weak memory, a generic notion of linearizability is difficult to
pin down~\cite{DongolJRA18,ifm18}. We therefore present a direct
technique for establishing contextual refinement under weak memory. A
key innovation is the development of context-sensitive simulation
rules that ensure that each client thread that uses the
implementation observes a subset of the values seen by the
abstraction. This is our second contribution.

% \noindent
% {\bf (3)} {\em Does the use of a library ever \emph{induce} client-side restrictions?}
% Under sequentially consistent memory, it is well known that the
% adherence to different correctness conditions induces different
% contextual guarantees. For example, the use of sequentially consistent
% libraries~\cite{DBLP:books/daglib/0020056} only guarantees contextual
% refinement when the client does not communicate outside of the
% libraries, whereas linearizable libraries are both necessary and
% sufficient if communication is
% allowed~\cite{DBLP:journals/tcs/FilipovicORY10}. In this paper, we
% explore this question in the context of weak memory, and show that
% proof rules can be simplified if we assume clients only synchronise
% through the libraries they use. This is our third contribution.

% \noindent
{\bf (3)} {\em Can the same abstract library specify \emph{multiple}
  implementations?}  A key benefit of refinement is the ability to use
the same abstract specification for multiple implementations, e.g., to
fine-tune clients for different concurrent workload scenarios. To
demonstrate the applicability of our framework, we provide a
proof-of-concept example for an abstract lock and show that the same
lock specification can be implemented by a sequence lock and ticket
lock. The theory itself is generic and can be applied to concurrent
objects in general; we prove correctness of the Treiber
Stack adapted for RC11-RAR. This is our third contribution.


% \noindent
{\bf (4)} {\em How can we support verification? Can the
  verification techniques be mechanised?}
Assuming the existence of an operational semantics for the underlying
memory model, we aim for \emph{deductive} verification of both
client-library composition and contextual refinement. We show that
this can be supported %by mechanisation
by prototyping the full verification stack in the Isabelle/HOL theorem
prover.\footnote{Our Isabelle theories may be accessed via~\cite{Isabelle}.}
This is our fourth contribution.

\smallskip  
\noindent{\bf Overview.}
In \refsec{sec:message-passing-via} we motivate the main ideas and
illustrate the basic principle of message-passing synchronisation, but
for programs comprising a program executing with an abstract
library. \refsec{sec:gener-weak-memory} presents a modular programming language
and operational semantics for reads/write accesses within this
language. A method for encoding the operational semantics of abstract
objects is given in \refsec{sec:abstr-object-semant}. In
\refsec{sec:example-verification}, we describe verification of client
programs that use abstract libraries, and in \refsec{sec:cont-refin}
we present our refinement theory. We use an abstract lock and two
different implementations of this lock as running examples. %  in
% Sections~\ref{sec:example-verification} and
% \ref{sec:cont-refin}. 
Finally, in \refsec{sec:view-based-relax}, we discuss the
specification of generic concurrent objects that exploit view-based
relaxations, making use of the framework developed in
\refsec{sec:abstr-object-semant}. Here, we also describe the
verification of the Treiber Stack adapted for C11.





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

